Haystack: A Multi-Purpose Mobile Vantage Point in User Space

Despite our growing reliance on mobile phones for a wide range of daily tasks, their operation remains largely opaque. A number of previous studies have addressed elements of this problem in a partial fashion, trading off analytic comprehensiveness and deployment scale. We overcome the barriers to large-scale deployment (e.g., requiring rooted devices) and comprehensiveness of previous efforts by taking a novel approach that leverages the VPN API on mobile devices to design Haystack, an in-situ mobile measurement platform that operates exclusively on the device, providing full access to the device's network traffic and local context without requiring root access. We present the design of Haystack and its implementation in an Android app that we deploy via standard distribution channels. Using data collected from 450 users of the app, we exemplify the advantages of Haystack over the state of the art and demonstrate its seamless experience even under demanding conditions. We also demonstrate its utility to users and researchers in characterizing mobile traffic and privacy risks.

==> Makefile <==
###########################################################
#
# Makefile for LaTeX docs
#

TEX = paper
FIGS = 
PSFIGS = $(FIGS:.pdf=.ps)

all: pdf
ps:  $(TEX).ps
pdf: $(TEX).pdf
dvi: $(TEX).dvi

clean:
	$(RM) *.out *.aux *.log *.bbl *.blg *~ \#*\# *.toc *.idx *.eps dummy
	$(RM) $(patsubst %.tex, %.ps, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.dvi, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.pdf, $(wildcard *.tex))

# only need -Ppdf if using CM fonts

paper.pdf: *.tex paper.bib Makefile
	pdflatex paper.tex
	bibtex paper
	pdflatex paper.tex
	pdflatex paper.tex

# This is for a tool of mine that monitors files for changes via
# inotify and then executes actions. --cpk
notif:
	notif -vv *.tex *.bib make

